HAWC Detection of a TeV Halo Candidate Surrounding a Radio-quiet pulsar

Extended very-high-energy (VHE; 0.1-100 TeV) $\gamma$-ray emission has been observed around several middle-aged pulsars and referred to as ``TeV halos". Their formation mechanism remains under debate. It is also unknown whether they are ubiquitous or related to certain subgroup of pulsars. With 2321 days of observation, the High Altitude Water Cherenkov (HAWC) Gamma-Ray Observatory detected VHE $\gamma$-ray emission at the location of the radio-quiet pulsar PSR J0359+5414 with $>6\sigma$ significance. By performing likelihood tests with different spectral and spatial models and comparing the TeV spectrum with multi-wavelength observations of nearby sources, we show that this excess is consistent with a TeV halo associated with PSR J0359+5414, though future observation of HAWC and multi-wavelength follow-ups are needed to confirm this nature. This new halo candidate is located in a non-crowded region in the outer Galaxy. It shares similar properties to the other halos but its pulsar is younger and radio-quiet. Our observation implies that TeV halos could commonly exist around pulsars and their formation does not depend on the configuration of the pulsar magnetosphere.

==> natbib.tex <==
\bibitem[Vianello et al.(2015)]{2015arXiv150708343V} Vianello, G., Lauer, R.~J., Younk, P., et al.\ 2015, arXiv:1507.08343
\bibitem[Vianello et al.(2015)]{2015arXiv150708343V} Vianello, G., Lauer, R.~J., Younk, P., et al.\ 2015, arXiv:1507.08343
\bibitem[Abeysekara et al.(2017)]{2017ApJ...843...39A} Abeysekara, A.~U., Albert, A., Alfaro, R., et al.\ 2017, \apj, 843, 39. doi:10.3847/1538-4357/aa7555

